BINGO-ABDUS: a radiotelescope to unveil the dark sector of the Universe

we review the Baryon Acoustic Oscillations from Integrated Neutral Gas Observations (BINGO) telescope, an international collaboration, led by Brazil and China, aiming to explore the Universe history through integrated post-reionization 21cm signals and fast radio emissions. For identifying individually fast radio sources, the Advanced Bingo Dark Universe Studies (ABDUS) project has been proposed and developed and will combine the current BINGO construction with the main single-dish telescope and stations of phased-array and outrigger.

==> newconfig/newsettings.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%for boxes
\definecolor{main}{HTML}{5989cf}    % setting main color to be used
\definecolor{sub}{HTML}{cde4ff}     % setting sub color to be used

\newtcolorbox{boxC}{
    colback = sub, % background color
    boxrule = 0pt  % no borders
}

\newtcolorbox{boxL}{
    fontupper = \color{main},
    rounded corners,
    arc = 6pt,
    colback = sub, 
    colframe = main!50, 
    boxrule = 0pt, 
    bottomrule = 4.5pt 
}

\newtcolorbox{boxM}{
    fontupper = \color{white},
    rounded corners,
    arc = 6pt,
    colback = main!80, 
    colframe = main, 
    boxrule = 0pt, 
    bottomrule = 4.5pt,
    enhanced,
    fuzzy shadow = {0pt}{-3pt}{-0.5pt}{0.5pt}{black!35}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

